Towards Truss-Based Temporal Community Search

Identifying communities from temporal networks facilitates the understanding of potential dynamic relationships among entities, which has already received extensive applications. However, existing methods primarily rely on lower-order connectivity (e.g., temporal edges) to capture the structural and temporal cohesiveness of the community, often neglecting higher-order temporal connectivity, which leads to sub-optimal results. To overcome this dilemma, we propose a novel temporal community model named maximal-truss (MDT). This model emphasizes maximal temporal support, ensuring all edges are connected by a sequence of triangles with elegant temporal properties. To search the MDT containing the user-initiated query node q (q-MDT), we first design a powerful local search framework with some effective pruning strategies. This approach aims to identify the solution from the small temporal subgraph which is expanded from q. To further improve the performance on large graphs, we build the temporal trussness index (TT-index) for all edges. Leveraging the TT-index allows us to efficiently search high-probability target subgraphs instead of performing a full search across the entire input graph. Empirical results on nine real-world networks and seven competitors demonstrate the superiority of our solutions in terms of efficiency, effectiveness, and scalability

==> draft-stub.tex <==

	%这里可以用平均的角度去推导
	% 最后再写这些，算法先理清楚
	%或者直接写成T^2 m的1.5次方
%	\begin{Theorem}
%		The construction of the \textit{TBT} index is $\mathcal{O}(|\bar {\mathcal E}|^{1.5}T)$.
%	\end{Theorem}
%	
%	%等图画出来再写
%	\begin{Proof}
%		From  a horizontal view, there are $|\mathcal E|/ T$ edges on average in each temporal subgraph in $\delta-slice$, and each edge participates in an average of $m^{0.5}$ triangles. There are $O(T)$ temporal subgraphs in $\delta-slice $, so the operation for updating temporal subgraphs and updating $TSup$ spend $T \times (|\bar {\mathcal E}|/ T + |\bar {\mathcal E}|/ T \times {|\bar {\mathcal E}}|^{0.5})=|\bar {\mathcal E}|+{|\bar {\mathcal E}}^{1.5}|$. Since $\delta $ varies from 0 to $T$, the time complexity of constructing $TBT$ index is $T\times(|\bar {\mathcal E}|+{|\bar {\mathcal E}|}^{1.5})$.
%	\end{Proof}
	
	%
	%\begin{Theorem}
	%	The construction of the \textit{TBT} index is $\mathcal{O}(|\bar {\mathcal E}|^{1.5}T^2$.
	%\end{Theorem}
	%
	%%等图画出来再写
	%\begin{Proof}
	%From  a horizontal view, for each temporal subgraph in $\delta-slice$, there are most $|\bar {\mathcal E}|$ edges and there are at most $|\bar {\mathcal E}|$ triangles need to update $TSup$. Therefore, the operation takes $T|\bar {\mathcal E}|$ time to get $TSup_{\delta}$. Since $\delta $ varies from 0 to $T$, the time complexity of constructing $TBT$ index is $\mathcal{O}(|\bar {\mathcal E}|^{1.5}T^2)$.
	%\end{Proof}
	%
	%
	%%把子图也表示进去，直接用两个累计和\sum\sum
	%\begin{Theorem}
	%	The construction of the \textit{TBT} index is $O(T \times {|\mathcal E|+\sum_{\bar e}()})$
	%\end{Theorem}
	%
	%%等图画出来再写
	%\begin{Proof}
	%	From  a horizontal view, for each temporal subgraph in $\delta-slice$, there are most $|\bar {\mathcal E}|$ edges and there are at most $|\bar {\mathcal E}|$ triangles need to update $TSup$. Therefore, the operation takes $T|\bar {\mathcal E}|$ time to get $TSup_{\delta}$. Since $\delta $ varies from 0 to $T$, the time complexity of constructing $TBT$ index is $\mathcal{O}(|\bar {\mathcal E}|^{1.5}T^2)$.
	%\end{Proof}
	
	% 师兄给的建议
	% 存储的应该是增量,先别写伪代码吧思路理顺再说.
	% 先写伪代码？可以写划分为子图，子图用起始顶点来标记（可以写为什么要划分为重叠的子图，因为这样才能列出所有的组合，这里可以给出证明画个图+证明）.
	
	% 师兄给的建议
	% 这段应该放在前面，介绍索引结构到底是什么样子的，分解成（delta，tau）这样的对，因为很可能存在delta增大，其temporal support 并没有改变的情况，我们提出了domain这个性质，同时按这个保存，并且保证他们是notdomained（为了节省空间），介绍一下分解的过程直接说和前面的shrink的过程很像，只不过是要查索引，维护他的domain性质，
	
	%之所以这些写,不直接add时态边是因为可以直接用一个变量
	% \If{$\bar{e}$ is not in $\mathcal{H}_{\delta}[t]$}
	% {
		
		% \For{$w$ in $\mathcal{D}_{\mathcal{H}_{\delta}[t]}(u) \cap \mathcal{D}_{\mathcal{H}_{\delta}[t]}(v)$}
		% {
			% $TSup_{\mathcal{H}_{\delta}[t]}(\triangle_{uvw})=0$
			% }
		% $\mathcal{D}_{\mathcal{H}_{\delta}[t]}(u).add(v)$;             $\mathcal{D}_{\mathcal{H}_{\delta}[t]}(v).add(u)$\;
		% \Else
		% {
			%     $\mathcal{H}_{\delta}[t].\bar{e}++$\;
			% }
		% }

%\begin{algorithm}[htb!]
%\caption{Count $\delta$-temporal triangle(CDT)} 	
%\label{alg:count_temp}
%	\KwIn{A temporal graph $\mathcal{G}$, a triangle $\triangle_{uvw}$ and an integer $\delta$.}
%    \KwOut{The number of $\delta$-temporal triangle.}
%    \BlankLine 
%    Initial $TSup_{\mathcal{G}}(\triangle_{uvw}, \delta)=0$\;
%    ${TS}_{uv}=\{t|(u,v,t)\in \mathcal{G}\}$, $TS_{uw}=\{t|(u,w,t)\in \mathcal{G}\}$, $TS_{vw}=\{t|(v,w,t)\in \mathcal{G}\}$\;
%    sort $TS_{uv}$, $TS_{uw}$, $TS_{vw}$ in ascending order by $t$, respectively\;
%    sort $TS_{uv},TS_{uw},TS_{vw}$ in ascending order by their size, and mark them as $TS_1,TS_2,TS_3$,respectively\;
%    Initial $\mathcal{W}_2(t_1)=[l_2,h_2], t_1=TS_1[0],l_2=h_2=0$; $\mathcal{W}_3(t_2)=[l_3,h_3],t_2=TS_2[0],l_3=h_3=0$\;
%    % l_3,h_3为空时等于W_3(t2-1)时的l_3和h_3。
%    \For{$i$ in $0$ upto $TS_1.size()$}
%    {  
	%        \For{$l_2' \gets{TS_2[l_2]}$ in $TS_2$}{\If{$|t_2-t_1|\leq \delta$}{$t_{l_2} \gets{t_2}$ ;\textbf{break;}}}
	%        \For{$t_2 \gets{TS_2[h_2]}$ in $TS_2$}{\If{$|t_2-t_1| > \delta$}{\textbf{break;}} $t_{h_2} \gets{t_2}$}
	%        \For{$t_2 \gets{TS_2[l_2]}$ {\rm upto} $TS_2[h_2]}$ in $TS_2$}
%        {
	%  			\If{ $\mathcal{W}_3(t_2).empty()$ and $t_2!=TS_2[0]$}
	%  			{
		%  				$l_3 \gets{\mathcal{W}_3(t_2).t_{l_3}}$\;
		%  				$h_3 \gets{\mathcal{W}_3(t_2).t_{h_3}}$\;
		%  			}
	%            \For{$t_3 \gets{\mathcal{W}_3(t_2).t_{l_3}}$ in $TS_3$}{\If{$|t_2-t_3|\leq \delta$ and $|t_1-t_3|\leq \delta$ }{$\mathcal{W}_3(t_2).t_{l_3} \gets{t2}$ \textbf{break;}}}
	%            \For{$t_3 \gets{\mathcal{W}_3(t_2).{t_{h_3}}}$ in $TS_3$}{\If{$|t_2-t_3| > \delta$ or $|t_1-t_3| > \delta$ }{\textbf{break;}} $\mathcal{W}_3(t_2).{t_{h_3}} \gets{t_2}$}
	%            $TSup_{\mathcal{G}}(\triangle_{uvw})=TSup_{\mathcal{G}}(\triangle_{uvw})+|\mathcal{W}_3(t_2)|$
	%        }
%    }
%    \Return{ $TSup_{\mathcal{G}}(\triangle_{uvw})$}
%\end{algorithm}


% \begin{algorithm}[htb!]
% \caption{Count $\delta$-temporal triangle (CDT)} 	
% \label{alg:count_temp}
% \KwIn{Temporal graph $\mathcal{G}$, $\triangle_{uvw}$ and integer $\delta$.}
% \KwOut{$TSup_{\mathcal G}(\triangle,\delta)$}
% \BlankLine 
% Let $TSup_{\mathcal{G}}(\triangle_{uvw})=0$,
% $T(u,v)=\{t|(u,v,t)\in \mathcal{G}\}$, $T(u,w)=\{t|(u,w,t)\in \mathcal{G}\}$, $T(v,w)=\{t|(v,w,t)\in \mathcal{G}\}$\;

% sort  $T(u,v),T(u,w),T(v,w)$  in ascending order by their size, and mark them as $T_1,T_2,T_3$,respectively\;
% Initial $\mathcal{W}_2(t_1)=\{t_{l_2},...,t_2, ..., t_{h_2}\}$, where $t_{l_2}=t_{h_2}=T_2[0]$, and $\mathcal{W}_3(t_2)=\{t_{l_3},..., t_3, ..., t_{h_3}\}$ where $t_{l_3}=t_{h_3}=T_3[0]$.

% \For{$t_1$ in $T_1$}
% {  
% 	\For{$t_2 \gets{t_{l_2}}$ in $T_2$}{\If{$|t_2-t_1|\leq \delta$}{$t_{l_2} \gets{t_2}$ ;\textbf{break;}}}
% 	\For{$t_2 \gets{t_{h_2}}$ in $T_2$}{\If{$|t_2-t_1| > \delta$}{\textbf{break;}} $t_{h_2} \gets{t_2}$}
% 	\For{$t_2 \gets{t_{l_2}}$ {\rm upto} $t_{h_2}$ in $T_2$}
% 	{
% 		\For{$t_3 \gets{\mathcal{W}_3(t_2).t_{l_3}}$ in $T_3$}{\If{$|t_2-t_3|\leq \delta$ and $|t_1-t_3|\leq \delta$ }{$\mathcal{W}_3(t_2).t_{l_3} \gets{t_2}$ \textbf{break;}}}
% 		\For{$t_3 \gets{\mathcal{W}_3(t_2).{t_{h_3}}}$ in $T_3$}{\If{$|t_2-t_3| > \delta$ or $|t_1-t_3| > \delta$ }{\textbf{break;}} $\mathcal{W}_3(t_2).{t_{h_3}} \gets{t_2}$}
% 		$TSup_{\mathcal{G}}(\triangle_{uvw})+=|\mathcal{W}_3(t_2)|$;
% 	}
% }
% \Return $TSup_{\mathcal{G}}(\triangle_{uvw})$;
% \end{algorithm}



%或者可以把countTempSup()这个程序放到CDT中
% \subsection{Global Method}
% As defined in Definition \ref{def:problem2}, the \textit{MDT} is actually a $(k^*,\delta)$-truss which maximizes the value of $k$. For a temporal graph $\mathcal{G}$ and a fixed $\delta$, the $(k,\delta)$-truss has the similar properties to $k$-truss, that is $(k,\delta)$-truss are included in $(k-1,\delta)$-truss. Inspired by this, we borrow some ideas from \textit{truss-decompose} \cite{DBLP:conf/sigmod/HuangCQTY14} and designed a global framework Algorithm \ref{alg:global} to find a \textit{MDT} solution. The main idea of Algorithm \ref{alg:global} is first to count the temporal support for all edge (lines 1-2) and then iteratively removing the edges with the lowest temporal support edges to attempt finding the $MDT$-like community from $(0,\delta)$-truss, $(1,\delta)$-truss,..., $(k^*-1,\delta)$-truss, and finally search $MDT$ community by checking the temporal triangle connectivity (line 4). In more details, 
% %Specifically, for a temporal graph $\mathcal{G}$, and a fixed $\delta$, having get the temporal support for each static edge in it, the $MDT$ problem has a close relation to $k$-truss \cite{DBLP:conf/sigmod/HuangCQTY14} , we borrow some ideas from it and designed a global framework Algorithm \ref{alg:global} to find a $MDT$ solution.
% in earlier Subsection \ref{sec:temp_trian_count}, we introduced the Algorihtm \ref{alg:count_temp} to count the number of $\delta$-temporal triangles that a static triangle can induce. 
% And according to Definition \ref{def:tsup}, the $\delta$-temporal support of an edge is the number of $\delta$-temporal triangles that it can participate in. In this way, given a $\delta$, to get the value of $TSup(\bar e)$ for each $\bar e(u,v) \in \bar{\mathcal G}$, we search all the triangles that $\bar e$ particpates in.
% % we first collect the node set $\triangle_{uv}=\{w| \exists(u,w,t_1),(v,w,t_2) \in \mathcal{E}\}$, which denotes all triangles that contain edge $\bar e(u,v)$.
% Then calculate and accumulate $TSup(\triangle_{uvw})$ for each $w\in \triangle_{uv}$ to get $TSup(\bar e)$ by employing the Procedure \textit{CountTSup} (lines 6-16). Having get the temporal support for each static edge, we employ Algorithm \ref{alg:shrink} to find the $MDT$-like community, which has optimal the lowest temporal support $k^*$.

% %As defined in Definition \ref{def:problem2}, the $MDT$ is a special $(k,\delta)$-truss that has the maximal value of $k$. In this way, for a fixed $\delta$, the $(k,\delta)$-truss has the similar properties to $k$-truss, that is $(k,\delta)$-truss are included in $(k-1,\delta)$-truss. Inspired by this, we can find a \textit{MDT} from the subgraph $H$ which contains query vertex $q$ and maximal the lowest temporal support of the edges in it. In this way, we can achieve this target by iteratively removing the edge with the least support. Specifically, the optimal process are named \textit{ShrinkPruning} and displayed in Algorithm \ref{alg:shrink}.

% \begin{algorithm}[htb]
% %\scriptsize 
% \caption{Global strategy for finding \textit{MDT} (\textit{GS})} 	\label{alg:global}
% \KwIn{Temporal graph $\mathcal{G}$, integer $\delta$ and node $q$}
% \KwOut{Temporal subgraphs $\mathcal S_1,...,S_i$.}
% \BlankLine 
% % Initial $Q=\emptyset$ as a priority queue (in ascending order)\; 
% \For{$\bar e(u,v)$ in $E$}{$CountTSup(\mathcal{G},\bar e,\delta)$;}
% $\mathcal H,k^*=ShrinkPruning(\mathcal{G},q)$\;
% $\mathcal S=Connecting(\mathcal{H},q)$\;
% \Return $\mathcal S$\;
% \BlankLine
% \textbf{Procedure}\ {$CountTSup$}(${\mathcal{G}},\bar e,\delta$)\\
% TrianVis=$\emptyset$\;
% \For{$\bar e(u,v)$ in $\mathcal G$}
% {
% 	Initial $TSup(\bar{e})=0$\;
% 	\If{$|\mathcal{D}(u)|>|\mathcal{D}(v)|$}{swap$(u,v)$;}
% 	\For{$w$ in $\mathcal{D}(u)$}
% 	{
% 		\If{$w$ is in $\mathcal{D}(v)$}
% 		{
% 			\If{$\triangle_{uvw}$ is not in TrianVis}
% 			{$CDT(\mathcal{G},\triangle_{uvw},\delta)$; $TrianVis \gets{TrianVis \cup{\triangle_{uvw}}};$}
% 			$TSup(\bar{e})=TSup(\bar{e})+TSup(\triangle_{uvw})$\;
% 		}
% 	}
% }
% \Return{$e.TSup$;}
% \BlankLine
% \textbf{Procedure}\ {$Connecting$}(${\mathcal{G}},q$)\\
% Initial $Q=\emptyset, \ i=0$, $vis=\emptyset$\;
% \For{$u$ in $\mathcal{D}(q)$}
% {
% 	$Q.push(\bar e(q,u))$, $\mathcal{S}_{++i}=\emptyset$\;
% 	\While{$!Q.empty()$}
% 	{
% 		$\bar{e}(u,v)=Q.front()$, $\mathcal{S}_i\gets{\mathcal{S}_i \cup{\bar e}}$\;
% 		\For{$w$ in $\mathcal D(u) \cap \mathcal D(v)$}
% 		{
% 			\If{$\triangle_{uvw}.TSup==0$}{continue;}
% 			\If{$\bar{e}_1(u,w)$ is not in vis}{$Q.push(\bar e_1);\ vis\gets{vis\cup{\bar{e}_1}}$}
% 			\If{$\bar{e}_2(u,w)$ is not in vis}{$Q.push(\bar e_2);\ vis\gets{vis\cup{\bar{e}_1}}$}
% 		}
% 	}
% }
% \Return{$\mathcal{S}_1,\mathcal{S}_2,...,\mathcal{S}_i$;}
% \end{algorithm}	


% Specifically, Algorithm \ref{alg:shrink} first defines a priority queue $Q$ to record the temporal support of all edges in ascending order of their temporal support (lines 2-4). 
% Then Algorithm \ref{alg:shrink} greedily removes the edge $\bar{e}(u,v)$ with the smallest temporal support, and destroys all triangles that $\bar{e}$ participates in. So, it is necessary to update the temporal support of the edges inside the same triangle as  $\bar{e}$ (Lines 13-21). This process terminates when the number of edge induced by $q$ is less than 2, denoted as $qedge<2$. Since $qedge<2$ indicates that $q$ will not be contained in any triangle, so that $q$ does not participate in any temporal triangles. So, the Algorithm \ref{alg:shrink} ensure that the residual subgraph $\mathcal H$ contains the query node $q$ and the temporal support of each edge is no less than $k^*$, where $k^*=\max_k$\{$k|q\in(k,\delta)$-truss\}. It is worth noting that when the algorithm stops, there may exist a “Greedy-Accident”, which means some edges are mistakenly deleted based on the greedy strategy, as they are deleted to try to explore the maximal subgraph whose lowest temporal support is $k^*+1$, but this community actually not exist. So, if and only if the Algorithm \ref{alg:shrink} successfully found a maximal subgraph which can optimal the lowest temporal support, we update it as the returned subgraph $\mathcal H$ (Line 6). However, such a temporal subgraph $\mathcal H$ may not a qualified $(k^*,\delta)-truss$ as its properties of temporal triangle connectivity are not guaranteed. Therefore, it is necessary to check its temporal triangle connectivity for the output temporal subgraph by Algorithm \ref{alg:shrink}. And thus we develop the procedure \textit{Connecting}, which starts with an edge $\bar{e}(q,v)$ that induced by query node $q$, and to find all edges that are temporal triangle connected with $\bar{e}$. Specifically, \textit{Connecting} first accesses the edges that contained in the same temporalisable triangle with $\bar{e}$, then add them to the solution and the queue $Q$ in order to continuously search. This procedure terminates when all the \textit{MDT}s are found and we proof its correctness as follows.


% \begin{algorithm}[htb]
% %\scriptsize 
% \caption{ShrinkPruning} 	\label{alg:shrink}
% \KwIn{Temporal graph $\mathcal{G}$, query vertex $q$.}
% \KwOut{A temporal subgraph $\mathcal{H}$ upand $k^*$.}
% \BlankLine 
% Initial qedge=$|\mathcal{D}(q)|$, EdgeVis=$\emptyset$, $H=\emptyset$, $k^*=0$\;
% $Q=\emptyset$ is a priority queue (in ascending order by temporal support)\; 
% \For{$\bar e(u,v)$ in $ {\mathcal G}$}{$Q.push({\bar{e}})$;}
% \While{$qedge\geq 2$}
% {
% $\mathcal{H}=\mathcal{G}$; $k^*=Q.front().TSup$\; 
% \While{$qedge\geq 2$}
% {
% 	$\bar{e}(u,v)=Q.front()$; $supl=\bar e.TSup$\;
% 	\If{$supl\geq k^*$}
% 	{
% 		EdgeVis $\gets{ EdgeVis \cup {\bar e}}$; \ $Q.pop()$\;
% 		remove $\bar e$ from $\mathcal{G}$\;
% 		\If{$u==q$ or $v==q$}{$qedge\gets{qedge-1}$;}
% 		\For{$w$ in $\mathcal D(u) \cap \mathcal D(v)$}
% 		{
% 			\If{$TSup(\triangle_{uvw})==0$}{\textbf {Continue;}}
% 			\If{$\bar e_2(u,w)$ is not in EdgeVis and $\bar e_3(v,w)$ is not in EdgeVis }
% 			{                                    \If{$Q(\bar e_2).TSup>k^*$}{$Q(\bar e_2).TSup -=TSup(\triangle_{uvw})$;}
% 				\If{$Q(\bar e_2).TSup>k^*$}{$Q(\bar e_2).TSup-=TSup(\triangle_{uvw})$;}
% 			}
% 		}
% 	}\Else{\Return {$\mathcal{H},\ k^*$};}
% }
% }
% \Return {$\mathcal{H},\ k^*$};
% \end{algorithm}	


% \begin{Proof}
% Suppose $\mathcal{H}$ is the output of Algorithm \ref{alg:shrink}, which contains $q$ and all edges $\bar{e}(u,v)\in \mathcal{H}$ satisfied that $TSup_{\mathcal{H}}(\bar{e})\geq{k^*}$. Obviously, according to Definition \ref{def:k-delta-truss}, $\mathcal{H}$ has fulfilled conditions (1) and (3). The Procedure \textit{Connecting} iteratively extends from the edge induced by $q$ to satisfy Condition (2), and it is clearly Condition (3) can still be met at the same time. So, the most important is to proof that all temproal subgraph $\mathcal{S}_i$ returned by \textit{Connecting} are still keep condition (1). For a $MDT$ denoted as $\mathcal{S}_i$, suppose triangle $\triangle_{uvw}\in \mathcal{H}$ , and edge $\bar{e^*}(u,v) \notin \mathcal{S}_i$ and $\bar{e}_1(u,w)\in \mathcal{S}_i$, that means $\triangle_{uvw}$ is non-temporalisable and there is no other temporalisable triangle $\triangle_{uvw_1}$ can connect $\bar{e^*}$ with $(u,w_1)\in \mathcal{S}_i$, which means that $TSup_{\mathcal{H}}(\bar{e}_1(u,w)=TSup_{\mathcal{S}_i}(\bar{e}_1(u,w))$. In this way , the correctness of Procedure \textit{Connecting} is promised.
% \end{Proof}
% % 不能加入到结果的边表明不能和已经子结果里面的边时态三角形连通，所有不会影响结果里面边的sup值。

% %\begin{Theorem}
% %The time complexity of \textit{GS} is $\mathcal{O}|\bar {\mathcal E}|^{1.5}T\delta^{2}$.
% %\end{Theorem}
% %
% %%算TSup时要访问好多个三角形的：这里得取个平均
% %\begin{Proof}
% %Procedure \textit{CountTempSup} first calls \textit{CDT} for each static triangle to compute the $TSup$ for each edge, there are at most $|\bar {\mathcal E}|^{1.5}$ triangles, so its time complexity is $\mathcal{O}(|\bar {\mathcal E}|^{1.5}T\delta^{2})$. Besides, \textit{ShrinkPrune} and \textit{Connecting} algorithms spend $|\bar {\mathcal E}|^{1.5}$ time to access all the edges. So the time complexity of \textit{GS} is $\mathcal{O}(|\bar {\mathcal E}|^{1.5}T\delta^{2})$.
% %\end{Proof}


% \begin{Theorem}
% The time complexity of \textit{GS} is $O(|\triangle_\mathcal{G}|T\delta^{2}+  |\bar {\mathcal E}| + \log{|\bar {\mathcal E}|}\sum_{\bar e(u,v)\in \bar {\mathcal E}}\min(|\mathcal{D}(u)|,|\mathcal{D}(v)|))$, where $|\triangle_{\mathcal G}|$ denotes the number of triangle in $\mathcal G$.
% \end{Theorem}

% %算TSup时要访问好多个三角形的：这里得取个平均
% \begin{Proof}
% Algorithm \ref{alg:global} first calls the Procedure \textit{CountTSup} to compute the $TSup$ for the edges. Clearly, for each edge $\bar e(u,v)$, \textit{CountTSup} takes $\min(|\mathcal{D}(u)|,|\mathcal{D}(u)|)$ time to identify the triangles. And for each triangle it calls Algorithm \ref{alg:count_temp} to count the temporal triangles. Therefore it spends $\sum_{\bar e(u,v)\in \bar {\mathcal E}}\min(|\mathcal{D}(u)|,|\mathcal{D}(v)|)+|\triangle_\mathcal{G}|T\delta^{2}$ to count the temporal support for all edges, $|\triangle_\mathcal{G}|$ denotes the number of the triangles in $\mathcal G$. Besides, it is clear that Algorithm \ref{alg:shrink} needs $O(\log{|\bar {\mathcal E}|}\sum_{\bar e(u,v)\in \bar {\mathcal E}}\min(|\mathcal{D}(u)|,|\mathcal{D}(v)|))$ to finish the delete and update operation. As for the \textit{Connecting} procedure, whose complexity is related to the size of the solutions which is no more than ${O}(|\bar {\mathcal E}|)$.
% \end{Proof}


% \begin{figure}[!htb]
% \begin{center}
% \subfigure[$(4,3)$-truss]{ 
% \label{fig:global_example:a} 
% \includegraphics[scale=0.12]{Fig/g_1.png} 
% } 
% \subfigure[$(5,3)$-truss]{ 
% \label{fig:global_example:b} %% label for first subfigure 
% \includegraphics[scale=0.12]{Fig/g_2.png} 
% } 

% \subfigure[$(8,3)$-truss]{ 
% \label{fig:global_example:c}
% \includegraphics[scale=0.12]{Fig/g_3.png} 
% } 
% \subfigure[$(12,3)$-truss]{ 
% \label{fig:global_example:d} %% label for second subfigure 
% \includegraphics[scale=0.12]{Fig/g_4.png} 
% } 

% \caption{\centering{The process of global search  strategy.}}
% \label{fig:global_example}
% \end{center}
%  \vspace{-0.7cm}
% \end{figure}

% \begin{Example}
% Given a temporal subgraph \ref{fig:basic_example:a}, and set $\delta=3$. \figurename\ref{fig:global_example} illustrates the search process of the global strategy. According to the Definition \ref{def:k-delta-truss}, since $\min\{Tsup_{\mathcal{G}}(\bar e)|\bar e \in \mathcal G\}=4$, the temporal graph $\mathcal{G}$ itself is a $(4,3)$-truss and $k^*=4$. As $qedge=6 \geq 2$, the algorithm iterately deletes the edges $\{\bar e(u,v)\leq 4|\bar e \in \mathcal G\}$, so the edges $\bar e(6,4)$, $\bar e(7,8)$ and $\bar e(6,7)$ are deleted, and the residual subgraphs is showed in \figurename\ref{fig:global_example:b}, which is a $(5,3)$-truss and $k^*=5$. In the next iteration, the algorithm deletes the edge $\bar e(1,6)$ and $\bar e(2,6)$ to get a $(8,3)$-truss in \figurename\ref{fig:global_example:c}.  And then the algorithm continue deleting the edges and obtaining the final solution $(12,3)$-truss in \figurename\ref{fig:global_example:d}. It is worth noting that the algorithm attempts to explore the solution in \figurename\ref{fig:global_example:d} by removing edges $\bar e(1,2)$, and it terminates because $supl<12$ (line 9 in Algorithm \ref{alg:shrink}). Therefore, the $(12,3)$-truss is the final solution.
% \end{Example}

% Obviously, the global Algorithm \ref{alg:global} needs to calculate the temporal support for all edges in $\mathcal{G}$ and then greedily delete the edges, which may be inefficient for massive temporal graphs as the unnecessary calculations. For example, some edges are not triangle connected with any edge induced by $q$, and they must not appear in the solution. But the global strategy still needs to compute their temporal support, and these edges induce larger input scales for Algorithm \ref{alg:shrink} and Procedure \textit{Connecting}, resulting in unnecessary calculations. In addition, taking the whole graph as the input for Algorithm \ref{alg:shrink}, the edges with too small temporal support may not included in the solution, but the global method still takes time to remove them. With these considerations in mind, we proposed a local search strategy in Section \ref{subsec:local} to overcome these shortcomings.
% % and take this check as \textit{Connect} procedure, which selects a $(k^*,\delta)-truss$ contained $q$ from $H$. Specifically, the \textit{Connect} procedure select edges from the edge induced by node $q$ and adds the edges to solution with 

% % check_connect可以写一个proof：证明这个样子是可以得到准确值的

% % 大概还是要写一个check connect的伪代码

% % \begin{algorithm}[htb!]
% % %\scriptsize 
% % \caption{Connect} 	\label{alg:connect}
% % 	\KwIn{The output of Algorithm \ref{alg:shrink}, query vertex $q$.}
% %     \KwOut{A maximal-$\delta-truss$ $\mathcal{S}$.}
% %     \BlankLine 
% %     \For{$u$ in $\mathcal{D}(u)$}
% %     {

% %     }
% %     \Return {$S$};
% % \end{algorithm}	

% and Table \ref{tab:index_example} displays the \textit{TBT}-index for the temporal subgraph in \figurename\ref{fig:basic_example:a}.
% \begin{table}[htb]
% 	%\renewcommand\arraystretch{1.4}
% 	\centering
% 	\caption{\textit{TBT} index for edges in $\mathcal G$ \figurename\ref{fig:basic_example:a}}
% 	\scalebox{1.0}{
% 		\begin{tabular}{c|l}
% 			\toprule
% 			Edge & \ $TBT[\bar e]$ \\
% 			\midrule
% 			$\bar e(1,2)$ & (1,3),(2,6),(3,12),(4,15),(5,18),(6,22),(7,24)\\
% 			$\bar e(1,3)$ & (1,3),(2,6),(3,12),(4,15),(5,18),(6,22),(7,24)\\
% 			$\bar e(1,4)$ & (1,2),(2,6),(3,12),(4,15),(5,18),(6,22),(7,24)\\
% 			$\bar e(1,5)$ & (1,2),(2,6),(3,12),(4,15),(5,18),(6,22),(7,24)\\
% 			$\bar e(2,3)$ & (1,3),(2,7),(3,12),(4,15),(5,18),(6,22),(7,24)\\
% 			$\bar e(2,4)$ & (1,2),(2,7),(3,12),(4,15),(5,18),(6,22),(7,24)\\
% 			$\bar e(2,5)$ & (1,2),(2,7),(3,12),(4,15),(5,18),(6,22),(7,24)\\
% 			$\bar e(3,4)$ & (1,3),(2,7),(3,12),(4,15),(5,18),(6,22),(7,24)\\
% 			$\bar e(3,5)$ & (1,3),(2,7),(3,12),(4,15),(5,18),(6,22),(7,24)\\
% 			$\bar e(4,5)$ & (1,3),(2,7),(3,12),(4,15),(5,18),(6,22),(7,24)\\
% 			$\bar e(1,6)$ & (1,2),(2,3),(3,5),(4,6),(5,8)\\
% 			$\bar e(1,7)$ & (1,2),(2,8)\\
% 			$\bar e(2,6)$ & (1,2),(2,3),(3,5),(4,6),(6,8)\\
% 			$\bar e(5,7)$ & (1,2),(2,8)\\
% 			$\bar e(6.7)$ & (2,2),(3,4),(4,7),(5,10),(6,12)\\
% 			$\bar e(6,8)$ & (2,1),(3,4),(4,7),(5,10),(6,12)\\
% 			$\bar e(7,8)$ & (2,1),(3,4),(4,7),(5,10),(6,12)\\
			
% 			\bottomrule
% 		\end{tabular}
% 	}
% \end{table}		

%
%Recall that we can employ \textit{CDT} procedure to compute the temporal support under a given $\delta$. Although the parameter $\delta$ theoretically has a wide range of values, 	
%	which employs Algorithm \ref{alg:count_temp} to compute the temporal support. Combining the Definition \ref{def:tsup}, which require that $\delta$ is an integer, 
%we can still find a reasonable upper bound for it. In fact, in the case 
	
%	

	
	% 算sup虽然可以自底向上利用底层信息，但是其实质上还是每一层在重新计算，我们试图找到一些sup的依赖关系，并且得到如下结论。
	% 接着就介绍新的proposition。或者说我们可以改写上面那个公式。

	% 虽然找到了关系但是没有找Tsup之间的关系，我们可以利用这个公式计算出每个\delta下每条边的sup值，但是进一步地我们
	
	% 这里可以有个例子画图来说明一下，然后还要引出增量的概念
	% 接下来写推论，增量式地计算而不用，怎么衔接还没想好
	% 我们的算法是横向和纵向相结合的，纵向更新，横向计算
	% 可以说一下，不用的部分就可以clear掉来减轻内存压力，内存空间可以证明一下
	%这里需要画个图来说明Tsup的计算过程

  %Totally, \figurename\ref{fig:index_example} shows the framework for constructing the \textit{TBT} index, and the complexity analysis of Algorithm \ref{alg:index_construct} is as follows.

		
%		\begin{equation}
%			\begin{aligned}
%				&  TSup_{\mathcal{G}}(\bar{e})= TSup_{\mathcal{G}}(\triangle_1)+ ... +TSup_{\mathcal{G}}(\triangle_j)+...+TSup_{\mathcal{G}}(\triangle_n) \\
%				&+TSup_{\mathcal{G}_{1}}(\triangle_1,\delta-1)+\sum_{i=1}^{t_{max}-\delta}(\Phi_{TSup_{\mathcal{G}_{[i,\delta+i]}}(\triangle_1,\delta)}-\Phi_{TSup_{\mathcal{G}_{[i,\delta+i-1]}}(\triangle_1,\delta-1)})\\
%				&+...\\
%				&+TSup_{\mathcal{G}_{1}}(\triangle_j,\delta-1)+ \sum_{i=1}^{t_{max}-\delta}(\Phi_{TSup_{\mathcal{G}_{[i,\delta+i]}}(\triangle_j,\delta)}-\Phi_{TSup_{\mathcal{G}_{[i,\delta+i-1]}}(\triangle_j,\delta-1)})\\
%				&+...\\
%				&+TSup_{\mathcal{G}_{1}}(\triangle_n,\delta-1)+ \sum_{i=1}^{\mathcal{G}.t_{max}-\delta}(\Phi_{TSup_{\mathcal{G}_{[i,\delta+i]}}(\triangle_n,\delta)}-\Phi_{TSup_{\mathcal{G}_{[i,\delta+i-1]}}(\triangle_n,\delta-1)})\\
%				&=TSup_{\mathcal{G}_1}(\bar{e},\delta-1)+\sum_{i=1}^{\mathcal{G}.t_{max}-\delta}(\Phi_{TSup_{\mathcal{G}_{[i,\delta+i]}}(\bar{e},\delta)}-\Phi_{TSup_{\mathcal{G}_{[i,\delta+i-1]}}(\bar{e},\delta-1)})
%			\end{aligned}
%		\end{equation}

	
%	
%	\begin{Proof}
%		According Definition \ref{def:tsup}, for an edge $\bar{e}\in \mathcal{G}$, the temporal support $TSup_{\mathcal{G}}(\bar{e})=\sum_{j=1}^{n}TSup_{\mathcal{G}}(\triangle_j)$, where $\triangle_j$ denotes the triangle contains $\bar{e}$, then we can get that
%		
%		\begin{equation}
%			\begin{aligned}
%				&  TSup_{\mathcal{G}}(\bar{e})= TSup_{\mathcal{G}}(\triangle_1)+ ... +TSup_{\mathcal{G}}(\triangle_j)+...+TSup_{\mathcal{G}}(\triangle_n) \\
%				&+TSup_{\mathcal{G}_{1}}(\triangle_1,\delta-1)+ \\ &\sum_{i=1}^{\mathcal{G}.t_{max}-\delta}(\Phi_{TSup_{\mathcal{G}_{[i,\delta+i]}}(\triangle_1,\delta)}-\Phi_{TSup_{\mathcal{G}_{[i,\delta+i-1]}}(\triangle_1,\delta-1)})\\
%				&+...\\
%				&+TSup_{\mathcal{G}_{1}}(\triangle_j,\delta-1)+\\ &\sum_{i=1}^{\mathcal{G}.t_{max}-\delta}(\Phi_{TSup_{\mathcal{G}_{[i,\delta+i]}}(\triangle_j,\delta)}-\Phi_{TSup_{\mathcal{G}_{[i,\delta+i-1]}}(\triangle_j,\delta-1)})\\
%				&+...\\
%				&+TSup_{\mathcal{G}_{1}}(\triangle_n,\delta-1)+\\ &\sum_{i=1}^{\mathcal{G}.t_{max}-\delta}(\Phi_{TSup_{\mathcal{G}_{[i,\delta+i]}}(\triangle_n,\delta)}-\Phi_{TSup_{\mathcal{G}_{[i,\delta+i-1]}}(\triangle_n,\delta-1)})\\
%				&=TSup_{\mathcal{G}_1}(\bar{e},\delta-1)+\\
%				&\sum_{i=1}^{\mathcal{G}.t_{max}-\delta}(\Phi_{TSup_{\mathcal{G}_{[i,\delta+i]}}(\bar{e},\delta)}-\Phi_{TSup_{\mathcal{G}_{[i,\delta+i-1]}}(\bar{e},\delta-1)})
%			\end{aligned}
%		\end{equation}
%	\end{Proof}
%	
	
	




%\newcounter{MYtempeqncnt}
%\begin{figure*}[!t]
%	% ensure that we have normalsize text
%	\normalsize
%	% Store the current equation number.
%	\setcounter{MYtempeqncnt}{\value{equation}}
%	% Set the equation number to one less than the one
%	% desired for the first equation here.
%	% The value here will have to changed if equations
%	% are added or removed prior to the place these
%	% equations are referenced in the main text.
%	\setcounter{equation}{5}
%	\begin{equation}
%		\label{eqn_dbl_x}
%		x = 5 + 7 + 9 + 11 + 13 + 15 + 17 + 19 + 21+ 23 + 25
%		+ 27 + 29 + 31
%	\end{equation}
%	\begin{equation}
%		\label{eqn_dbl_y}
%		y = 4 + 6 + 8 + 10 + 12 + 14 + 16 + 18 + 20+ 22 + 24
%		+ 26 + 28 + 30
%	\end{equation}
%	% Restore the current equation number.
%	\setcounter{equation}{\value{MYtempeqncnt}}
%	% The IEEE uses as a separator
%	\hrulefill
%	% The spacer can be tweaked to stop underfull vboxes.
%	\vspace*{4pt}
%\end{figure*}

%实验部分experiment.tex
%
%\begin{table*}[t!] 
%	\centering
%	\caption{Running Time for Different Temporal Methods (ms) }
%% 	\vspace{-0.2cm}
%	\scalebox{1.35}{
	%		\begin{tabular}{c|rrrrrrrr}
		%			\toprule
		%			Dataset & OL & PCore & DCCS  & FirmCore & L-MEGA & GS &LS &IS \\
		%			\midrule
		%			 Rmin & 47121  &769308  & *   & 4112281   &2420     & 577   &469  & 3\\ 
		%			 Primary &69515  & 11463 & 4094 & 959   &160203     &924  &352 &5 \\
		%		     Lyon &1635670   & 38524712 &19335 & 3587   &787731    &50560  &48514 &831 \\
		%			 Thiers & 2077790  &10603183  &175428  & 16084  &290311   &56754 &26501 & 379\\ 	 
		%			Twitter & 353517 &66362   &8323   &26036       &*   &7887 &444 &56 \\
		%	        Facebook & 51213 &28967205  &3796355  & 2413352   & *    &4435 & 206 &18 \\
		%			Enron & 267906  &  153909163  &491361   &2073825   &*     &27515 &4489 &283 \\ 
		%	    	Lkml & 3130130  & 159965765  & 1638877  &44882      &*      &79022  &16547 &839 \\ 
		%		    DBLP & 2435710  & 185330 & 5236058  &8080973       &*    &446099 &339240 &40660 \\ 
		%		    AVG.RANK & 6 & 7 &4  &5  &8 &3  &2  & 1 \\
		%		\bottomrule		
		%			\end{tabular}}
%	\label{tab:running_time_for_various_method}
%% 	\vspace{-0.7cm}
%\end{table*} 


% Fig/dblp_varyts.pdf

% \begin{figure*}[h]
% \begin{minipage}{0.65\linewidth}
% % \setlength{\abovecaptionskip}{5mm}
% \caption{Effectiveness for Different Temporal Methods }
% \label{tab:effec_various_method}
% \scalebox{0.78}{
% \begin{tabular}{c|crrrrrrrr}
% 			\toprule
% 			\multicolumn{2}{c}{}
% 			&k-truss &MAPPR & OL & PCore & DCCS  & FirmCore & L-MEGA & MDT \\
% 			\midrule
% 			\multirow{9}*{   \textit{HTD}   }
% 			&Rmin & 0.00007   &  0.00089   &  0.00498  &  0.00176   & *  & 0.00414 & 0.00021     &  0.01106   \\ 
% 			&Primary & 0.00479   &  0.03768   & 0.13751   & 0.0461    &  0.15874    & 0.0221    & 0.0669  & 0.1609\\
% 			&Lyon & 0.02038   &  0.09283   & 0.14888   &  0.78574   & 0.09654     & 0.1   & 0.00021 &  0.1426\\
% 			&Thiers & 0.00925   &  0.04642   & 0.12805   &  0.09655   &  0.08434    & 0.04516    & 0.01963 & 0.13751 \\ 	 
% 			&Twitter &  0.0008  &  0.001   & 0.34056   & 0.00341    & 0.11696     & 0.08879    & *  &0.36365  \\
% 			&Facebook & 0.01016   &  0.00001   & 0.01508   &0.15081     & 0.1  & 0.00001    &*  & 0.07368  \\
% 			&Enron & 0.00025   & 0.00685    & 0.01804   & 0.00241    & 0.00001     & 0.00418    &*  &0.14095   \\ 
% 			&Lkml & 0.06299   & 0.18989    & 0.26226   & 0.13408    & 0.01125     & 0.16105    &* & 0.52042  \\ 
% 			&DBLP & 0.39787   & 0.57478    & 0.6401   & 0.51182    & 0.22405     & 0.54407    &*  &0.80436   \\ 
% 			&AVG.RANK &7    & 5    & 2   &    3 &  4    &  6   &8  & 1 \\
% 			\midrule
% 			\multirow{9}*{   \textit{HTC}   }
% 			&Rmin & 1   & 0.73225    &0.90037    &0.67877  &*   &0.67787  &0.7211      & 0.57939    \\ 
% 			&Primary &0.79225    & 0.56849    & 0.97105   & 0.52811    & 0.80813  & 0.86898 &  0.54241    & 0.7802\\
% 			&Lyon & 1   &  0.83441   &0.95451    &0.90039  & 0.99767  & 0.97431 & 0.75084 &0.91382 \\
% 			&Thiers & 1   &  0.78531   & 0.75383   & 0.98391    & 0.9391  & 0.9966 & 0.68487 &0.66646  \\ 	 
% 			&Twitter &0.74328    & 0.70028    & 0.96348   & 0.77779    &0.92273   &0.9314  & *     &0.65159  \\
% 			&Facebook & 0.6932   & 0.676    & 0.69151   & 0.69329    &0.25791   &0  &*      &0.66891  \\
% 			&Enron &0.82007    & 0.68761    & 0.98123   & 0.96308    & 0.8645  &0.89774  & *   & 0.60762 \\ 
% 			&Lkml &  0.99698  & 0.87261    &0.99189    & 0.93365    &0.90057   & 0.90263 & *     & 0.81753 \\ 
% 			&DBLP & 0.51533   & 0.66011    & 0.77391   & 0.81835    & 0.8868  &0.03288  &* & 0.64509 \\ 
% 			&AVG.RANK & 7   & 3    & 8   &5     &6      &4     &2  &1  \\   
% 			\bottomrule	
% \end{tabular}}
% \end{minipage}
% \begin{minipage}{0.3\linewidth}
% \setlength{\abovecaptionskip}{-0.5mm}
% \subfigbottomskip=-1pt
% \subfigcapskip=-5pt
% \flushright{\caption{Scalability}
% }
%  \label{fig:sca}
%    \flushright{
%    \subfigure[DBLP (vary $|V|$)]{ 
% 		\label{fig:sca:varyn} 
% 		\includegraphics[scale=0.20]{Fig/dblp_varyn.pdf} 
% 	}}
  
% \flushright{
%    \subfigure[DBLP (vary $TS$)]{ 
% 		\label{fig:sca:varyts} 
% 		\includegraphics[scale=0.20]{Fig/dblp_varyts.pdf} 
% 	}}  
%  % \flushright{\caption{Scalability}}
%  % \label{fig:sca}
% \end{minipage}
%     % \hfill
%     % \caption{figure and table}
%     % \label{zrotate}
% \end{figure*}

